Neural Estimation for Scaling Entropic Multimarginal Optimal Transport

Multimarginal optimal transport (MOT) is a powerful framework for modeling interactions between multiple distributions, yet its applicability is bottlenecked by a high computational overhead. Entropic regularization provides computational speedups via the multimarginal Sinkhorn algorithm, whose time complexity, for a dataset size $n$ and $k$ marginals, generally scales as $O(n^k)$. However, this dependence on the dataset size $n$ is computationally prohibitive for many machine learning problems. In this work, we propose a new computational framework for entropic MOT, dubbed Neural Entropic MOT (NEMOT), that enjoys significantly improved scalability. NEMOT employs neural networks trained using mini-batches, which transfers the computational complexity from the dataset size to the size of the mini-batch, leading to substantial gains. We provide formal guarantees on the accuracy of NEMOT via non-asymptotic error bounds. We supplement these with numerical results that demonstrate the performance gains of NEMOT over Sinkhorn's algorithm, as well as extensions to neural computation of multimarginal entropic Gromov-Wasserstein alignment. In particular, orders-of-magnitude speedups are observed relative to the state-of-the-art, with a notable increase in the feasible number of samples and marginals. NEMOT seamlessly integrates as a module in large-scale machine learning pipelines, and can serve to expand the practical applicability of entropic MOT for tasks involving multimarginal data.

==> figures/barchart.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{gray119}{RGB}{119,119,119}
\definecolor{steelblue52138189}{RGB}{52,138,189}

\begin{axis}[
axis background/.style={fill=gainsboro229},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel=\textcolor{dimgray85}{b},
xmajorgrids,
xmin=-0.6625, xmax=5.6625,
xtick style={color=dimgray85},
xtick={0,1,2,3,4,5},
xticklabels={32,64,128,256,512,1028},
y grid style={white},
ylabel=\textcolor{dimgray85}{Values},
ymajorgrids,
ymin=0, ymax=18.165,
ytick style={color=dimgray85}
]
\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:-0.375,0) rectangle (axis cs:-0.125,7.33);
\addlegendimage{ybar,ybar legend,draw=none,fill=chocolate2267451,very thin}
% \addlegendentry{k_3}

\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:0.625,0) rectangle (axis cs:0.875,3.78);
\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:1.625,0) rectangle (axis cs:1.875,1.9);
\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:2.625,0) rectangle (axis cs:2.875,1.05);
\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:3.625,0) rectangle (axis cs:3.875,0.62);
\draw[draw=none,fill=chocolate2267451,very thin] (axis cs:4.625,0) rectangle (axis cs:4.875,0.27);
\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:-0.125,0) rectangle (axis cs:0.125,12.1);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue52138189,very thin}
% \addlegendentry{k_4}

\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:0.875,0) rectangle (axis cs:1.125,5.59);
\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:1.875,0) rectangle (axis cs:2.125,3.07);
\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:2.875,0) rectangle (axis cs:3.125,1.76);
\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:3.875,0) rectangle (axis cs:4.125,0.81);
\draw[draw=none,fill=steelblue52138189,very thin] (axis cs:4.875,0) rectangle (axis cs:5.125,0.44);
\draw[draw=none,fill=gray119,very thin] (axis cs:0.125,0) rectangle (axis cs:0.375,17.3);
\addlegendimage{ybar,ybar legend,draw=none,fill=gray119,very thin}
% \addlegendentry{k_5}

\draw[draw=none,fill=gray119,very thin] (axis cs:1.125,0) rectangle (axis cs:1.375,8.6);
\draw[draw=none,fill=gray119,very thin] (axis cs:2.125,0) rectangle (axis cs:2.375,4.3);
\draw[draw=none,fill=gray119,very thin] (axis cs:3.125,0) rectangle (axis cs:3.375,2.3);
\draw[draw=none,fill=gray119,very thin] (axis cs:4.125,0) rectangle (axis cs:4.375,1.2);
\draw[draw=none,fill=gray119,very thin] (axis cs:5.125,0) rectangle (axis cs:5.375,0.6);
\end{axis}

\end{tikzpicture}


==> figures/mnist.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{steelblue52138189}{RGB}{52,138,189}
\definecolor{springgreen60179113}{RGB}{50,149,94}


\begin{axis}[
width=5cm, height=4cm,
legend style={at={(0.985,0.05)}, anchor=south east , fill opacity=0.65, draw opacity=1, text opacity=1, draw=none},
axis background/.style={fill=gainsboro229},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
% xmode=log,
% ymode= log,
xlabel=\textcolor{dimgray85}{$k$},
xmajorgrids,
xmin=2.3, xmax=9.5,
xtick={3,4,5,6,7,8,9},
xtick style={color=dimgray85},
y grid style={white},
ylabel=\textcolor{dimgray85}{OT loss},
ymajorgrids,
% ymin=1.260153970691875, ymax=1.77164667469609,
ymin=1.4, ymax=4,
ytick style={color=dimgray85},
ylabel style={yshift=-10pt}
]
\addplot [steelblue52138189, mark=*, mark size=3, mark options={solid}]
table {%
9	3.815
8	3.4252
7	3.0625
6	2.7391
5	2.3486
4	2.016
3	1.649
};

% \addlegendentry{NEMOT (ours)}
% \addlegendentry{Sinkhorn}
% \addlegendentry{Neural Estimator - Simplified}
\end{axis}

\end{tikzpicture}

